Coresets remembered and items forgotten: submodular maximization with deletions

In recent years we have witnessed an increase on the development of methods for submodular optimization, which have been motivated by the wide applicability of submodular functions in real-world data-science problems. In this paper, we contribute to this line of work by considering the problem of robust submodular maximization against unexpected deletions, which may occur due to privacy issues or user preferences. Specifically, we consider the minimum number of items an algorithm has to remember, in order to achieve a non-trivial approximation guarantee against adversarial deletion of up to $d$ items. We refer to the set of items that an algorithm has to keep before adversarial deletions as a deletion-robust coreset. Our theoretical contributions are two-fold. First, we propose a single-pass streaming algorithm that yields a $(1-2\epsilon)/(4p)$-approximation for maximizing a non-decreasing submodular function under a general p-matroid constraint and requires a coreset of size $k + d/\epsilon$, where $k$ is the maximum size of a feasible solution. To the best of our knowledge, this is the first work to achieve an (asymptotically) optimal coreset, as no constant-factor approximation is possible with a coreset of size sublinear in $d$. Second, we devise an effective offline algorithm that guarantees stronger approximation ratios with a coreset of size $O(d \log(k)/\epsilon)$. We also demonstrate the superior empirical performance of the proposed algorithms in real-life applications.

==> legacy/alg-sieve.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
\KwIn{parameter \Cgap}
%\KwOut{Ouput}
$\topd \gets \emptyset, \topv \gets 0, \C \gets \emptyset$\;
Initialize $\I_\thr=\emptyset$ for any $\thr \in \reals$\;
\For{$v \in \V$}{
	$\topd \gets \topd + v$ 
	\tcp*{preserve top $\nD+1$ singletons in \topd}
	\lIf{$|\topd| \le \nD+1$}{
		\Continue
	}
	$v \gets \arg\min_{u \in \topd} f(u), \topd \gets \topd - v, \topv \gets \max\{f(v), \topv\}$\;
	$\thrs \gets \{ (1+\Cgap)^i: \frac{\topv}{2\nI(1+\Cgap)}\le (1+\Cgap)^i \le \topv \}$\;
	$\C \gets \C + v$\;
	Remove from \C all items $v$ such that $f(v \mid \I_\thr) < \thr$ for every $\thr \in \{\thr' \in \thrs: |\I_{\thr'}| < \nI \}$
	\label{step:sieve-remove}\;
	\lIf{$|\C| < \nD/\Cgap$}{
		\Continue
	}
	Sample an item $v$ from \C with probability proportional to $1 / f(v \mid \I_{\thr(v)})$,
	where $\thr(v) = \max \{\thr \in \thrs: |\I_\thr| < \nI, f(v \mid \I_\thr) \ge \thr \}$ \;
	$\I_{\thr(v)} \gets \I_{\thr(v)} + v$\;
}
\Return{$\{ \I_\thr \}_{\thr \in \thrs}$, \topd and \C}
\caption{Robust \sieve algorithm}
\label{alg-sieve}
\end{algorithm}

\begin{algorithm}[t]
\DontPrintSemicolon
\KwIn{$\{ \I_\thr \}_{\thr \in \thrs}$, \topd, \C, and \D}
%\KwOut{Ouput}
$\R \gets \topd + \C + \cup_{\thr \in \thrs} \I_\thr$\;
$\topv' \gets \max_{v \in \R \setminus \D} f(v)$\;
$\thrs' \gets \{ (1+\Cgap)^i: \frac{\topv'}{2\nI(1+\Cgap)}\le (1+\Cgap)^i \le \topv' \}$ \;
\For{$\thr \in \thrs'$}{
	$S_\thr \gets \I_\thr$ if $\thr \in \thrs$; 
	otherwise $S_\thr \gets \emptyset$\;
	\For{$v \in \R \setminus \D$}{
		\If{$|S_\thr| < \nI$ and $f(v \mid S_\thr) \ge \thr$}{
			$S_\thr \gets S_\thr + v$
		}
	}
}
\Return{$\arg\max_{S_\thr': \thr \in \thrs'} f(S_\thr')$ where $S_\thr' = S_\thr \setminus \D$}
\caption{Construction of \sieve solution after deletion}
\label{alg-sieve-after}
\end{algorithm}

==> legacy/cardinality.tex <==

\citet{badanidiyuru2014streaming} propose a streaming algorithm (\sieve) for non-decreasing submodular maximization under a cardinality constraint.
The \sieve algorithm maintains multiple tentative solutions, each of which is associated with an increasing threshold, and admits a new item only if its marginal gain is at least the threshold.
We develop a robust version of \sieve algorithm, displayed in Algorithm~\ref{alg-sieve}.
The algorithm simply inserts a randomized buffer between the data stream and a slightly modified \sieve algorithm, in which an arriving item is only assigned to the tentative solution with the largest threshold.
\note{The reason \sieve assigns a new item $v$ to all tentative solutions is to make the algorithm parallelizable.}

\input{legacy/alg-sieve}

We denote by a coreset \R the union of all items returned by Algorithm~\ref{alg-sieve}.
It is easy to see that the coreset size is at most $\bigO(\nI \log(\nI)/\Cgap + \nD/\Cgap)$.
In the rest of this section,
we prove that it is indeed robust.

We first state several useful results about the \sieve algorithm.

\begin{lemma}
There exists a threshold $\thr^* \in \thrs'$ enumerated by Algorithm~\ref{alg-sieve-after} such that 
$2\nI \thr^* \le f(\OPT) \le (1+\Cgap) 2\nI \thr^*$.
\end{lemma}
\begin{proof}
This can be ensured as long as we keep in \R the top singleton in $\V \setminus \D$.
Algorithm~\ref{alg-sieve} ensures this by keeping the top $\nD+1$ singletons in \topd.
\end{proof}

\begin{lemma}
For any threshold $\thr \in \thrs'$ enumerated by Algorithm~\ref{alg-sieve-after}, 
if $|\I_\thr| < \nI$,
we have
$f(v \mid \I_\thr) < \thr$ for any item $v \in \V \setminus \R$.
\end{lemma}
\begin{proof}
This is clear by noticing that the only step we discard an item $v \in \V \setminus \R$ is at Step~\ref{step:sieve-remove} in Algorithm~\ref{alg-sieve}.
\end{proof}

\begin{lemma}
$f(S_{\thr^*}) \ge (1-\epsilon) f(\OPT) /2$.
\end{lemma}
\begin{proof}
If $|S_{\thr^*}| = \nI$, we are done, because $f(S_{\thr^*}) \ge \nI \thr^* \ge f(\OPT)/2(1+\Cgap)$.
We discuss the case $|S_{\thr^*}| < \nI$ below.

Let $O$ be the optimal solution over data $\V' = (\V \setminus \R) + (\R \setminus \D)$.
Since $\OPT \subseteq \V \setminus \D \subseteq \V'$, we have $f(\OPT) \le f(O)$.

Algorithm~\ref{alg-sieve} and Algorithm~\ref{alg-sieve-after} can be seen as two stages of one \sieve algorithm.
That is, they start with $S_{\thr^*} = \emptyset$, process every item $v \in \V'$, and add $v$ into $S_{\thr^*}$ when $f(v \mid S_{\thr^*}) \ge \thr^*$.
Thus, 
\[
	f(O) \le f(O + S_{\thr^*}) 
	\le f(S_{\thr^*}) + \sum_{v \in O \setminus S_{\thr^*}} f(v \mid S_{\thr^*})
	\le f(S_{\thr^*}) + \nI \thr^*
	\le f(S_{\thr^*}) + f(\OPT)/2
	\le f(S_{\thr^*}) + f(O)/2.
\]
\end{proof}

What is left is to show that solution $S_{\thr^*}$ is robust against deletions.
We show this by first proving that $I_{\thr^*} \subseteq S_{\thr^*}$ is robust.
\begin{lemma}
\label{lemma:sieve-robust}
For any threshold $\thr \in \thrs'$ in Algorithm~\ref{alg-sieve-after}, we have
$\expect[f(\I_\thr')] \ge (1-\Cgap) \expect[f(\I_\thr)]$, 
where $\I_\thr' = \I_\thr \setminus \D$.
\end{lemma}
\begin{proof}
Write $\I = \I_\thr$ and $\I' = \I_\thr'$.
We denote by $\I_j$ the set of first $j-1$ items added into $\I$, and $\I_{j+1} = \I_j + v_j$.
\begin{align}
	\expect[f(\I')] 
	&\ge \expect[\sum_{j} f(v_j \mid \I_j) \indicator[v_j \not\in \D] ] \\
	&= \expect[\sum_{j} f(v_j \mid \I_j) (1 - \indicator[v_j \in \D]) ] \\
	&\ge (1 - \frac{|\D|}{\nD/\Cgap}) \expect[\sum_{j} f(v_j \mid \I_j)] \\
	&\ge (1 - \Cgap) \expect[f(\I)].
\end{align}
\note[flawed]{Items in the candidate set \C are not all assigned to $\I_\thr$, while the adversary only needs to target those that are assigned to $\I_{\thr^*}$.}
\end{proof}






